Dense Feature Learning via Linear Structure Preservation in Medical Data

Deep learning models for medical data are typically trained using task specific objectives that encourage representations to collapse onto a small number of discriminative directions. While effective for individual prediction problems, this paradigm underutilizes the rich structure of clinical data and limits the transferability, stability, and interpretability of learned features. In this work, we propose dense feature learning, a representation centric framework that explicitly shapes the linear structure of medical embeddings. Our approach operates directly on embedding matrices, encouraging spectral balance, subspace consistency, and feature orthogonality through objectives defined entirely in terms of linear algebraic properties. Without relying on labels or generative reconstruction, dense feature learning produces representations with higher effective rank, improved conditioning, and greater stability across time. Empirical evaluations across longitudinal EHR data, clinical text, and multimodal patient representations demonstrate consistent improvements in downstream linear performance, robustness, and subspace alignment compared to supervised and self supervised baselines. These results suggest that learning to span clinical variation may be as important as learning to predict clinical outcomes, and position representation geometry as a first class objective in medical AI.

==> dummy.tex <==

\textbf{Contributions.} We make the following contributions:
\begin{enumerate}[leftmargin=*]
    \item \textit{Timestamp-aligned cross-modal pretraining for wearables.} We introduce a simple, architecture-agnostic contrastive objective that uses \emph{strict same-timestamp} positives across PPG/ACC and in-batch negatives, learning physiologically consistent joint embeddings without labels.
    \item \textit{Modality-specific encoders with lightweight fusion.} Two ResNet1D towers (one per modality) produce projected embeddings that are fused with a small head (e.g., gated concatenation or conditional modulation) to retain modality-specific information while enabling interaction.
    \item \textit{Night-long downstream sequence modeling.} A Mamba-based sequence model consumes fused per-epoch embeddings to yield per-epoch predictions over an entire night, capturing long-range context that per-epoch heads cannot.
    \item \textit{Comprehensive evaluation for 4-class staging.} With subject-independent splits, we compare against supervised-from-scratch and unimodal baselines, and perform ablations over fusion mechanisms and sequence models (per-epoch MLP, BiLSTM, TCN vs.\ Mamba). We further analyze robustness to motion intensity and missing-modality inference (using only PPG or only ACC at test time).
\end{enumerate}


